Value-Incentivized Preference Optimization: A Unified Approach to Online and Offline RLHF

Reinforcement learning from human feedback (RLHF) has demonstrated great promise in aligning large language models (LLMs) with human preference. Depending on the availability of preference data, both online and offline RLHF are active areas of investigation. A key bottleneck is understanding how to incorporate uncertainty estimation in the reward function learned from the preference data for RLHF, regardless of how the preference data is collected. While the principles of optimism or pessimism under uncertainty are well-established in standard reinforcement learning (RL), a practically-implementable and theoretically-grounded form amenable to large language models is not yet available, as standard techniques for constructing confidence intervals become intractable under arbitrary policy parameterizations. In this paper, we introduce a unified approach to online and offline RLHF -- value-incentivized preference optimization (VPO) -- which regularizes the maximum-likelihood estimate of the reward function with the corresponding value function, modulated by a $\textit{sign}$ to indicate whether the optimism or pessimism is chosen. VPO also directly optimizes the policy with implicit reward modeling, and therefore shares a simpler RLHF pipeline similar to direct preference optimization. Theoretical guarantees of VPO are provided for both online and offline settings, matching the rates of their standard RL counterparts. Moreover, experiments on text summarization and dialog verify the practicality and effectiveness of VPO.

==> MAB.tex <==
\subsection{Synthetic bandit problems} 
 
We evaluate the proposed methods on two synthetic problems: i) a multi-armed bandit problem, and ii) a linear contextual bandit problem.
\paragraph{Multi-armed bandit (MAB) problem.} In this scenario, we set $|\mathcal{X}| = 1$ and $|\mathcal{Y}| = 10$.  For each $y\in\mathcal{Y}$, the ground truth reward $r^\star(x, y)$ is randomly generated i.i.d. from a uniform distribution $U([0, 1])$. The policy is parameterized by $\pi_{\theta}(\cdot|x) = \mathsf{softmax}(\theta(x,\cdot))$, where $\theta\in\mathbb{R}^{10}$. The reference policy $\pi_{\text{ref}}$ is set to $\pi_{\theta_{\text{ref}}}$ with $\theta_{\text{ref}}(x, y)$ sampled i.i.d. from $U([0, 1])$. 
\paragraph{Linear contextual bandit problem.} Here, we set $\mathcal{X} = \mathbb{R}^2$, $|\mathcal{Y}| = 50$. For each $(x, y)$ pair, the ground truth reward is given by $r^\star(x, y) = \left\langle\phi(x, y), \theta^\star\right\rangle$, where $\theta^\star\in\mathbb{R}^{10}$ is randomly sampled from $U([0, 1])$, and the feature vector $\phi(x, y)$ is the output of the hidden layer of a fixed two-layer MLP, with the input given by the concatenation of $x$ and the one-hot encoding of $y$. The activation function is set to tanh. The context vector $x$ is drawn from standard normal distribution. We focus on log-linear policy class $\pi_\theta(\cdot|x) = \mathsf{softmax}(\langle\theta, \phi(x, \cdot)\rangle)$, and set $\pi_{\text{ref}} = \pi_{\theta_{\text{ref}}}$ with $\theta_{\text{ref}}(x, y)$ sampled i.i.d. from $U([0, 1])$. 

For both problem we set $\pi_{\text{ref}} = \pi_{\mathsf{b}}= \dnorm$ and use mini-batch sample of size 5 in every iteration. We approximately solve the optimization problems by performing $20$ AdamW optimization steps with learning rate $0.01$ and weight decay rate $0.01$ in every iteration for the online setting and $1000$ steps for the offline setting.  

We plot the average results over 10 independent runs for both experiments in Figure~\ref{fig:synthetic_online} and Figure~\ref{fig:synthetic_offline}. As demonstrated in the left panel of Figure~\ref{fig:synthetic_online}, an appropriate choice of $\alpha$ allows our method to outperform the model-based MAB with MLE baseline in the long-term performance of cumulative regret, at the cost of slightly increased cumulative regret in the first 100 iterations. This highlights the effectiveness of the \algabb in achieving more principled exploration-exploitation trade-off.  In the right panel, it is evident that the MLE baseline struggles with principled exploration in the more complex linear contextual bandit problem, while our method is able to achieve sub-linear regret growth. For the offline setting, Figure~\ref{fig:synthetic_offline} demonstrates that the performance of both MLE-MAB and \algabb improves as the number of offline data increases. However, \algabb achieves a consistently lower sub-optimality gap compared with that of MLE-MAB.
%
\begin{figure*}[ht]
    \centering
%    \vspace{-4mm}
    \begin{tabular}{cc}
   \includegraphics[width=0.46\textwidth]{simple.pdf} &  \includegraphics[width=0.46\textwidth]{linear.pdf} 
    \end{tabular}
 %   \vspace{-4mm}
    \caption{The cumulative regret v.s. number of iterations plot of \algabb and MLE-MAB methods in the online MAB problem (left panel) and online linear contextual bandit problem (right panel), respectively. 
    }

    \label{fig:synthetic_online}
\end{figure*}

\begin{figure*}[ht]
    \centering
%    \vspace{-4mm}
    \begin{tabular}{cc}
   \includegraphics[width=0.46\textwidth]{simple_offline.pdf} &  \includegraphics[width=0.46\textwidth]{linear_offline.pdf} 
    \end{tabular}
 %   \vspace{-4mm}
    \caption{The sub-optimality gap v.s. number of data plot of \algabb and MLE-MAB methods in the offline MAB problem (left panel) and offline linear contextual bandit problem (right panel), respectively. 
    }

    \label{fig:synthetic_offline}
\end{figure*}

